Boolean Reasoning-Based Biclustering for Shifting Pattern Extraction

Biclustering is a powerful approach to search for patterns in data, as it can be driven by a function that measures the quality of diverse types of patterns of interest. However, due to its computational complexity, the exploration of the search space is usually guided by an algorithmic strategy, sometimes introducing random factors that simplify the computational cost (e.g. greedy search or evolutionary computation). Shifting patterns are specially interesting as they account constant fluctuations in data, i.e. they capture situations in which all the values in the pattern move up or down for one dimension maintaining the range amplitude for all the dimensions. This behaviour is very common in nature, e.g. in the analysis of gene expression data, where a subset of genes might go up or down for a subset of patients or experimental conditions, identifying functionally coherent categories. Boolean reasoning was recently revealed as an appropriate methodology to address the search for constant biclusters. In this work, this direction is extended to search for more general biclusters that include shifting patterns. The mathematical foundations are described in order to associate Boolean concepts with shifting patterns, and the methodology is presented to show that the induction of shifting patterns by means of Boolean reasoning is due to the ability of finding all inclusion--maximal {\delta}-shifting patterns. Experiments with a real dataset show the potential of our approach at finding biclusters with {\delta}-shifting patterns, which have been evaluated with the mean squared residue (MSR), providing an excellent performance at finding results very close to zero.

==> 010_shifting_patterns.tex <==
\todo[author=MM]{Shifting patterns literature review}

==> 02_Biclustering.tex <==




==> 99Harmonic_analysis.tex <==
Let us consider the square input data for biclustering (in general, not necessary constant, shifting, or scaling pattern induction). The idea of calculating the harmonic mean of bicluster width and height to rank better smaller square biclusters than wide but single--row or single--column. 

However, in our data there is a big disproportion between number of rows (9) and number of columns (112).  That means, that this measure value will be the same for any of found patterns as specified below.

\begin{table}[ht!]
    \centering
    \begin{tabular}{|c|c|c|}\hline
         rows (r) & columns (c) & $\frac{2}{\frac{1}{r}+\frac{1}{c}}$ \\ \hline
         4 & 4 & 4 \\
         3 & 6 & 4 \\
         6 & 3 & 4 \\ \hline
    \end{tabular}
    \caption{Caption}
    %\label{tab:my_label}
\end{table}

In my opinion the third one becomes much more similar to single--column pattern as it represents 66\% of conditions with only 2.6\% of genes.

The intuitive way of solving this issue is to made the averaged values to be data width and height dependent --- the percentage of data width and percentage of data height. In case of non--square data the measure stops to be the reflexive one. 

Let us assume, that the mentioned patterns were found in data of 8 rows and 16 columns. Than we may define the percentage of rows ($p_r$) percentage of columns ($p_c$) represented by the bicluster and find the value of the new harmonic average:

\begin{table}[ht!]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}\hline
         rows (r) & columns (c) & $\frac{2}{\frac{1}{r}+\frac{1}{c}}$ & $p_r$ & $p_c$ & $\frac{2}{\frac{1}{p_r}+\frac{1}{p_c}}$\\ \hline
         4 & 4 & 4 & $\frac{1}{2}$ & $\frac{1}{4}$ & $\frac{1}{3} = 0.(3)$\\
         3 & 6 & 4 & $\frac{3}{8}$ & $\frac{6}{16}$ & $\frac{36}{96} = 0.375$\\
         6 & 3 & 4 & $\frac{6}{8}$ & $\frac{3}{16}$ & $\frac{36}{120} = 0.3$\\ \hline
    \end{tabular}
    \caption{Caption}
    %\label{tab:my_label}
\end{table}

We may observe, that from the ranking point of view the second pattern is placed higher than two other as it extends the gene direction.
